Training Object Detectors from Few Weakly-Labeled and Many Unlabeled Images

Weakly-supervised object detection attempts to limit the amount of supervision by dispensing the need for bounding boxes, but still assumes image-level labels on the entire training set. In this work, we study the problem of training an object detector from one or few images with image-level labels and a larger set of completely unlabeled images. This is an extreme case of semi-supervised learning where the labeled data are not enough to bootstrap the learning of a detector. Our solution is to train a weakly-supervised student detector model from image-level pseudo-labels generated on the unlabeled set by a teacher classifier model, bootstrapped by region-level similarities to labeled images. Building upon the recent representative weakly-supervised pipeline PCL, our method can use more unlabeled images to achieve performance competitive or superior to many recent weakly-supervised detection solutions.

==> ext-plots.tex <==
\usepackage{tikzextern}
\usepackage{pgffor}
\newcommand{\extfig}[2]{\tikzsetnextfilename{fig/extern/#1}{#2}}
\newcommand{\extdata}[1]{}


==> no-plots.tex <==
\newcommand{\extfig}[2]{!!!}
\newcommand{\extdata}[1]{}


==> plots.tex <==
% main packages
\usepackage{tikz}
\usetikzlibrary{arrows,shapes,calc,matrix,fit,backgrounds}
\usepackage{pgfplots}
\usepackage{pgfplotstable}
\pgfplotsset{compat=1.9}

% other packages
% \usepackage{chapterfolder}
\usepackage{xstring}

%------------------------------------------------------------------------------
% externalization: requires defining \finalcopy first

\usepgfplotslibrary{external}
\tikzexternalize
% \tikzexternalize[prefix=fig/extern/]
\newcommand{\extfig}[2]{\tikzsetnextfilename{fig/extern/#1}{#2}}
\newcommand{\extdata}[1]{\input{#1}}
% \IfBeginWith*{\jobname}{fig/extern/}{\finalcopy}{}

%-----------------------------------------------------------------------------
% tikz styles

\tikzstyle{tight} = [inner sep=0pt,outer sep=0pt]

%-----------------------------------------------------------------------------
% pgfplots general options

% \newcommand{\plot}[2]{\cffolderinput{#1}{#2}}
% \newcommand{\data}[1]{\cfcurrentfolder #1.txt}
\newcommand{\tabread}[2]{\pgfplotstableread{\data{#1}}#2}

\newcommand{\leg}[1]{\addlegendentry{#1}}
% \newcommand{\legtext}[1]{\addlegendimage{empty legend} \addlegendentry{#1}}

\tikzset{every mark/.append style={solid}}
\pgfplotsset{%smooth,
	grid=both, width=\columnwidth, try min ticks=5,
% 	every axis x label/.style={at={(ticklabel cs:0.5)},anchor=north},
% 	every axis y label/.style={at={(ticklabel cs:0.5)},rotate=90,anchor=south},
	every axis/.append style={font=\scriptsize},
	every axis plot/.append style={thick,mark=none,mark size=1.2,tension=0.18},
	legend cell align=left, legend style={fill opacity=0.8},
}

\pgfplotsset{
	dash/.style={mark=o,dashed,opacity=0.7},
	dott/.style={mark=o,dotted,opacity=0.7},
}
\newcommand{\kilo}[1]{\thisrow{#1}/1000}
\newcommand{\perc}[2]{\thisrow{#1}/#2}
\newcommand{\map}[1]{\thisrow{#1}*100}

